ControlMath: Controllable Data Generation Promotes Math Generalist Models

Utilizing large language models (LLMs) for data augmentation has yielded encouraging results in mathematical reasoning. However, these approaches face constraints in problem diversity, potentially restricting them to in-domain/distribution data generation. To this end, we propose ControlMath, an iterative method involving an equation-generator module and two LLM-based agents. The module creates diverse equations, which the Problem-Crafter agent then transforms into math word problems. The Reverse-Agent filters and selects high-quality data, adhering to the "less is more" principle, achieving better results with fewer data points. This approach enables the generation of diverse math problems, not limited to specific domains or distributions. As a result, we collect ControlMathQA, which involves 190k math word problems. Extensive results prove that combining our dataset with in-domain datasets like GSM8K can help improve the model's mathematical ability to generalize, leading to improved performances both within and beyond specific domains.

==> tables/datasets.tex <==



  \begin{table}[h]
% \vspace{-10pt}
\small
    % \hfill
    % \begin{minipage}{0.45\textwidth}
        \centering
        
        \begin{tabular}{l|cc}
        \midrule
        Datasets& GSM8K&SVAMP \\
           \midrule
            Need Seed-Question? & 42.4 & 38.3 \\
            Pairs & 49.3 &46.8 \\
            \ModelNameC-7B & \textbf{50.8}&\textbf{49.3} \\
            \midrule
            LLaMA 2-13B & 51.0 & 50.9 \\
            \ModelNameP-13B & 55.5 &52.1 \\
            \ModelNameC-13B & \textbf{56.6}&\textbf{56.6} \\
               \midrule
            LLaMA 1-33B & 50.0 & 49.0 \\
            \ModelNameP-33B & \textbf{56.0} &\textbf{52.5}  \\
            \ModelNameC-33B & 53.7&51.5 \\
\bottomrule
        \end{tabular}
        \caption{Model performances on English datasets.}
        \label{gsm8k}
       \vspace{-10pt}
    % \end{minipage}
  \end{table}  
